MICO: Selective Search with Mutual Information Co-training

In contrast to traditional exhaustive search, selective search first clusters documents into several groups before all the documents are searched exhaustively by a query, to limit the search executed within one group or only a few groups. Selective search is designed to reduce the latency and computation in modern large-scale search systems. In this study, we propose MICO, a Mutual Information CO-training framework for selective search with minimal supervision using the search logs. After training, MICO does not only cluster the documents, but also routes unseen queries to the relevant clusters for efficient retrieval. In our empirical experiments, MICO significantly improves the performance on multiple metrics of selective search and outperforms a number of existing competitive baselines.

==> prelim.tex <==
% \textcolor{red}{(we need to give some education to readers what mutual information is and what information processing theory is)}

% In this paper, we only consider the empirical distribution of the data. Therefore, all the random variables are discrete.
We introduce the notations and the basic concept of mutual information briefly here.
We denote a random variable $X$'s probability function by $p_X(x)$. We shorten it to $p(x)$ or $p_X$ when its meaning is clear under its context. We use $p^\theta(x)$ when $p(x)$ is in a parametric distribution family and $\theta$ is the parameter.
$p_{XY}(x,y)$ is the joint distribution of two random variables $X$ and $Y$, and $p_{X|Y}(x|y)$ is the conditional distribution of $X$ given $Y$, while 
% There are two basic properties: $p_{XY}(x,y) = p_{X|Y}(x|y) p_Y(y)$, $p_Y(y) = \sum_{x\in\mathcal{X}} p_{XY}(x,y)$. 
$p_Y(y)=\sum_{x} p_{XY}(x,y)$ is the marginal distribution of $Y$ under $p_{XY}(x,y)$. 
% , i.e., the two properties are written as $p(x,y) = p(x|y) p(y)$, $p(y) = \sum_{x} p(x,y)$. 
% We use $x\sim p_X$ to denote that the distribution of $x$ is $p_X$. 
The expectation of a function $f(x)$ w.r.t. a random variable $x$ is defined by $\mathbb{E}_{x\sim p_X} [f(x)] = \sum_{x\in\mathcal{X}} f(x) p_X(x)$. 
% Therefore, we also have $p(y)=\mathbb{E}_{x\sim p_X} [p(y|x)]$. 
% In the rest of this paper, we ignore the subscripts of the probability functions and the support in the summation when their actual meaning is clear by the context.
% \subsection{Mutual information}
We denote the entropy of $X$ by $H(X) = H(p_X) = \mathbb{E}_{x\sim p_X} [-\log (p_X(x))]$, 
while the conditional entropy is $H(Y|X) = \mathbb{E}_{x\sim p_X} H(p_{Y|X}) =\mathbb{E}_{(x,y)\sim p_{XY}}[-\log (p_{Y|X})]$.
% The Kullback–Leibler (KL) divergence between $X$ and $X'$ is $D_{\mathrm{KL}}(X\|X') = \mathbb{E}_X \left[\log \left(\frac{p_{X}(x)}{p_{X'}(x)}\right)\right]$. 
The cross-entropy between $X$ and $X'$ is defined as $H(X;X') = \mathbb{E}_{x\sim p_X} [-\log (p_{X'}(x))]$. 
% The KL-divergence is commonly used as an objective function since $D_{\mathrm{KL}}(X\|X')$ is minimized when $p_X=p_{X'}$. 
% To make statements clearer, we also use $p_X$ in these entropy notations. 
We denote the mutual information between $X$ and $Y$ by $I(X;Y)=\sum_x \sum_y p_{XY} \log\left( \frac{p_{XY}}{p_X p_Y}\right)=H(X)-H(X|Y)$. It is minimized at 0 when $X$ and $Y$ are independent, i.e., $p_{XY}=p_X p_Y$. The chain rule for mutual information is $I(X;(Y,Z))=I(X;Z)+I(X;Y|Z)$ where $I(X;Y|Z)=H(X|Z)-H(X|Y,Z)\geq 0$.


